RAN Slicing in Multi-MVNO Environment under Dynamic Channel Conditions

With the increasing diversity in the requirement of wireless services with guaranteed quality of service(QoS), radio access network(RAN) slicing becomes an important aspect in implementation of next generation wireless systems(5G). RAN slicing involves division of network resources into many logical segments where each segment has specific QoS and can serve users of mobile virtual network operator(MVNO) with these requirements. This allows the Network Operator(NO) to provide service to multiple MVNOs each with different service requirements. Efficient allocation of the available resources to slices becomes vital in determining number of users and therefore, number of MVNOs that a NO can support. In this work, we study the problem of Modulation and Coding Scheme(MCS) aware RAN slicing(MaRS) in the context of a wireless system having MVNOs which have users with minimum data rate requirement. Channel Quality Indicator(CQI) report sent from each user in the network determines the MCS selected, which in turn determines the achievable data rate. But the channel conditions might not remain the same for the entire duration of user being served. For this reason, we consider the channel conditions to be dynamic where the choice of MCS level varies at each time instant. We model the MaRS problem as a Non-Linear Programming problem and show that it is NP-Hard. Next, we propose a solution based on greedy algorithm paradigm. We then develop an upper performance bound for this problem and finally evaluate the performance of proposed solution by comparing against the upper bound under various channel and network configurations.

==> Sections/old_Related_Works.tex <==
\section{Related Works}

There has been significant work to address the problem of RAN slicing, especially in the recent past. There have been many excellent surveys on this topic by several research communities ~\cite{8320765,8334921}. The authors in these surveys provide an excellent insight to the RAN slicing problem without delving into details. In all the recent works, the RAN resource sharing problem (addressed as RAN slicing problem~\cite{inproceedings,7926919,8253541}) has been dealt by designing solutions using various theoretical means {optimization~\cite{7926923}, game theory~\cite{article_Radio}}.

One of the key limitation of these works is that it does not show the actual deployment of RAN slices on top of a physical network. Although the authors in the paper~\cite{d2019slice} discuss RAN slicing policies and enforcement problem by considering fine grained control of resources, it falls short when we bring in dynamic channel conditions. Moreover, the problem formulation considers slice as allocation of certain percentage of resource blocks from a given pool without considering the underlying requirement for these slices.

One of the work which closely focuses on addressing RB allocation problem is~\cite{8407021}. The authors propose a RB partitioning algorithm which focuses on allocating RB to every MVNO by simultaneously maximizing the percentage of satisﬁed MVNOs while allocating the minimum amount of RB. However, the problem in~\cite{8407021} does not take into account the dynamic channel conditions.

Our work can be closely compared to \cite{8761163}. The authors of \cite{8761163} address the problem of RAN slicing by considering dynamic channel conditions in a SD-RAN based architecture. One of the key architectural differences between our work and \cite{8761163} is the flexibility supported for the MVNO in the SD-RAN architecture. In \cite{8761163}, the authors consider individual slice managers for each slice but a common scheduler for all the users. This provides very less flexibility for MVNOs. In our work, we consider independent scheduler for all MVNOs. This allows MVNO, the option of choosing its users for scheduling at each time interval. Section III discusses this in detail.

The papers~\cite{article,5678740} present a framework for LTE virtualization. The authors propose an architecture for virtualizing the LTE base stations (called eNodeB (eNB) in LTE architecture) with the objective of having different operators sharing the same physical resources. The solution is based on a hypervisor (as in CPU virtualization), which hosts different virtual nodes, allocates the resources and is responsible of the spectrum sharing and data multiplexing. And, In~\cite{6240347} the framework from ~\cite{article,5678740} is used to present a algorithm for scheduling physical RB for the virtual nodes. The main idea of this algorithm is that if a eNB is overloaded and a neighbor eNB has available resources, a user is selected to be migrated to the unloaded eNB. Although the concept of centralized control is similar to our work, the problem statement is completely different. In our work, we are addressing the problem of RAN slicing in a multi-MVNO environment as opposed to resource sharing.

In~\cite{7891795}, the authors discuss the problem we are addressing in this paper briefly while discussing different approaches of RAN slicing. But, they have not formally defined the problem and provided solution.

In summary, our work addresses the shortcomings of these papers by providing more flexibility to the MVNOs, developing efficient slicing algorithm with dynamic channel conditions and carrying out a thorough validation. 
